Spotting AI's Touch: Identifying LLM-Paraphrased Spans in Text

AI-generated text detection has attracted increasing attention as powerful language models approach human-level generation. Limited work is devoted to detecting (partially) AI-paraphrased texts. However, AI paraphrasing is commonly employed in various application scenarios for text refinement and diversity. To this end, we propose a novel detection framework, paraphrased text span detection (PTD), aiming to identify paraphrased text spans within a text. Different from text-level detection, PTD takes in the full text and assigns each of the sentences with a score indicating the paraphrasing degree. We construct a dedicated dataset, PASTED, for paraphrased text span detection. Both in-distribution and out-of-distribution results demonstrate the effectiveness of PTD models in identifying AI-paraphrased text spans. Statistical and model analysis explains the crucial role of the surrounding context of the paraphrased text spans. Extensive experiments show that PTD models can generalize to versatile paraphrasing prompts and multiple paraphrased text spans. We release our resources at https://github.com/Linzwcs/PASTED.

==> tables/global_indicator.tex <==
\begin{table}[t!]
    \centering
    \small
    \setlength{\tabcolsep}{4pt} % Adjust the 4pt value as needed
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model} & \textbf{AUROC} & \textbf{Accuracy}\\
        \midrule
        Classification & \textbf{0.95} & 74.85\% \\
        R-lexical & 0.93 & 79.33\% \\
        R-grammatical & 0.93 & 78.87\% \\
        R-syntactic & 0.92 & 80.44\% \\
        R-aggregate & 0.94 & \textbf{82.98\%} \\
        \bottomrule
    \end{tabular}
    \caption{
    \label{tab:global_indicator}
    Paraphrased text-span detection as a global paraphrasing indicator.
    }
    
\end{table}

==> tables/ood.tex <==

\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.05} 
% \setlength{\tabcolsep}{1.1pt}


\begin{tabular}{lcccc}

\toprule
\textbf{Model} & \textbf{AUROC} & \textbf{Detection Accuracy} & \textbf{Lexical Correlation} & \textbf{Syntactic Correlation} \\
\midrule
Classification  & 0.9382 & 0.4690 & 0.5978 & 0.6426 \\
\midrule
Regression (lexical div.)& 0.9411 & 0.4237 & 0.6476 & 0.6872\\
% \midrule
% Regression (lexical-4-gram) & & & & \\
\midrule
Regression (POS div.)& 0.9274 & 0.1875 & 0.6405 & 0.6666  \\
% \midrule
% Regression (POS-4-gram) & & & & \\
\midrule
Regression (Syntactic div.) & 0.8996 & 0.0901 & 0.5814 & 0.6297\\
% \midrule
% Regression (Syntactic-5-depth) & & & & \\
\midrule
% Regression (Semantic div.)& 0.8942 & 0.1559 & 0.5553 & 0.5672 \\
% \midrule
Regression (Multi-dimension) & 0.9343 & 0.1944 & 0.6441 & 0.6819\\
\bottomrule
\label{tab:main}
\end{tabular}
\caption{
 OOD
}
\end{table*}


==> tables/para_diff.tex <==
\begin{table}[t!]
    \centering
    \small
    \begin{tabular}{lc}
        \toprule
        \textbf{Data Source} & \textbf{AUROC} \\
        \midrule
        w/o Para.& 0.99 \\
        w/ Machine Para. & 0.98 \\
        w/ Human Para. & 0.85 \\
        w/ Machine/Human Para. & 0.92 \\
        \bottomrule
    \end{tabular}
    \caption{}
    \label{tab:para_diff}
\end{table}

==> tables/stat_div.tex <==

% 38.0


\begin{table}[t!]
    \centering
    \small
    \begin{tabular}{lcc}
        \toprule
         \textbf{Data} & $\mathbf{D}_{lex}$$\uparrow$  &  $\mathbf{D}_{syn}\uparrow$  \\
        \midrule
        \multicolumn{3}{c}{\textbf{Data Source}}\\
        \midrule
        Human-authored Raw.  & 27.91  & 30.96\\
        Machine-authored Raw. & 29.73 & 30.90\\
        \midrule
        \multicolumn{3}{c}{\textbf{Paraphrasing Method}}\\
        \midrule
         Context-aware Para. & 28.92 & 28.84\\
        Context-agnostic Para. & 29.42 & 32.61\\
        \bottomrule
    \end{tabular}
    \caption{}
    \label{tab:stat_div}
\end{table}

==> tmp.tex <==
\begin{table*}[t!]
\centering
    \begin{tabular}{llllll}
    \toprule
        Model & $AUROC$ & $Recall_P$ & $Recall_N$ & $AvgRe$c & $ACC$ \\
    \midrule
    text classification & - & - & - & - & - \\
    sentence classification & 0.9888 & 0.9628 & 0.9417 & 0.9523 & 0.9471 \\
    sentence regression (1gram BLEU) & 0.9863 & 0.951 & 0.9476 & 0.9493 & 0.948 \\
    sentence regression (4gram BLEU) & 0.9872 & 0.9463 & 0.9526 & 0.94945 & 0.9521 \\
    sentence regression (POS 4gram BLEU) & 0.9869 & 0.9585 & 0.9318 & 0.9451 & 0.9352 \\
    sentence regression (lexical diversity) & 0.9648 & - & - & - & 0.9312 \\
    sentence regression (syntax diversity) & 0.9845 & 0.9539 & 0.9229 & 0.9384 & 0.9501 \\
    \bottomrule
    \end{tabular}
    \centering
    \caption{Span Labeling Performances}
    \label{tab:sample}
\end{table*}


\begin{table*}[t!]
\centering
    \begin{tabular}{lllll}
    \toprule
        Model & $AUROC$ & $Recall_P$ & $Recall_N$ & $AvgRe$c  \\
    \midrule
    text classification & 0.9662 & 0.93 & 0.86 & 0.897 \\
    sentence classification & 0.9732 & 0.93 & 0.92 & 0.92 \\
    sentence regression (1gram BLEU) & 0.9624 & 0.92 & 0.90 & 0.91 \\
    sentence regression (4gram BLEU) & - & - & - & - \\
    sentence regression (POS 4gram BLEU) & - & - & - & - \\
    sentence regression (lexical diversity) & - & - & - & - \\
    sentence regression (syntax diversity) & - & - & - & - \\
    \bottomrule
    \end{tabular}
    \centering
    \caption{Text Classification Performances}
    \label{tab:sample}
\end{table*}
